FaaS Execution Models for Edge Applications

In this paper, we address the problem of supporting stateful workflows following a Function-as-a-Service (FaaS) model in edge networks. In particular we focus on the problem of data transfer, which can be a performance bottleneck due to the limited speed of communication links in some edge scenarios and we propose three different schemes: a pure FaaS implementation, StateProp, i.e., propagation of the application state throughout the entire chain of functions, and StateLocal, i.e., a solution where the state is kept local to the workers that run functions and retrieved only as needed. We then extend the proposed schemes to the more general case of applications modeled as Directed Acyclic Graphs (DAGs), which cover a broad range of practical applications, e.g., in the Internet of Things (IoT) area. Our contribution is validated via a prototype implementation. Experiments in emulated conditions show that applying the data locality principle reduces significantly the volume of network traffic required and improves the end-to-end delay performance, especially with local caching on edge nodes and low link speeds.

==> tables/comparison.tex <==
\begin{tabularx}{\textwidth}{X*{3}{p{0.2\textwidth}}}
    \hline

    \thead{Index} &
    \thead{Pure FaaS} &
    \thead{State propagation} &
    \thead{Local state} \\

    \hline

    Amount of data generated &
    High, esp.\ with large argument/return value & 
    High, esp.\ with large application state &
    Lowest \\
    \hline

    Maintaining state consistency &
    Easiest, client-centric &
    Requires some care, esp.\ on failures &
    Most complex due to ownership delegation to edge nodes \\
    \hline

    Readiness level &
    Can be implemented on today's serverless platforms &
    Only requires chaining support &
    Requires new elements (state keepers) and change to APIs \\
    \hline

    Can take advantage of previous executions &
    No &
    No &
    Yes \\
    \hline
\end{tabularx}
